Sensitivity Analysis of High-Dimensional Models with Correlated Inputs

Sensitivity analysis is an important tool used in many domains of computational science to either gain insight into the mathematical model and interaction of its parameters or study the uncertainty propagation through the input-output interactions. In many applications, the inputs are stochastically dependent, which violates one of the essential assumptions in the state-of-the-art sensitivity analysis methods. Consequently, the results obtained ignoring the correlations provide values which do not reflect the true contributions of the input parameters. This study proposes an approach to address the parameter correlations using a polynomial chaos expansion method and Rosenblatt and Cholesky transformations to reflect the parameter dependencies. Treatment of the correlated variables is discussed in context of variance and derivative-based sensitivity analysis. We demonstrate that the sensitivity of the correlated parameters can not only differ in magnitude, but even the sign of the derivative-based index can be inverted, thus significantly altering the model behavior compared to the prediction of the analysis disregarding the correlations. Numerous experiments are conducted using workflow automation tools within the VECMA toolkit.

==> 03MarketLP.tex <==
\section{Energy Market Model \label{sec:LPmodel}}
%LP model describing power grid and exchange of energy, approximation of integer variables.
%The unit commitment problem~\cite{Huang2017} in energy management aims to find the optimal power production schedule while meeting various system-wide constraints. It is a non-convex, large-scale mixed-integer programming problem that must be repeatedly solved in very limited time frames. 

%{\color{red} ED, not OPF, zones in continental europe and flow limits between the countries}
The European electricity market~\cite{ElectricityMarkets} is based on bidding zones, which are modeled as one node. Lossless ED considers a problem where the objective is to find the set of generator dispatch points  $\pg$ that minimize the total cost of meeting a specified demand $\pd$, without modeling any network infrastructure. The problem consists of several zones, where each zone contains several generators $\bfG$ and energy that can be imported or exported. Similarly, the problem is defined over a multiperiod time horizon $\bfT$.
The LP model in this work represents a simplified UC problem formulated as a continuous problem in order to have certain guarantees about the convergence and optimality of the solution, as well as  reducing the computation time. The LP model reads
\begin{linenomath}
\begin{subequations}
\label{LP}
\begin{align}
	& \minimize{\pg}  \quad \sum_{t \in \bfT} \sum_{g\in \bfG} \bfc^f_{g,t}  \pg_{g,t} \label{LP:obj}\\
	&\subject{}  \; \forall t \in \{ 1, 2, \ldots, N\}: \nonumber \\
	\label{LP:pg}
	& \pgen_{g,t} = \pgen_{g,t-1}+\pni{, \text{on}}{g,t}-\pni{, \text{off}}{g,t},\\
	\label{LP:balance}
	& \sum_{g\in \bfG} {\pgen}_{g,t} + \bfn^v_{t} + \psdni{}{t} = \pd_t + \pscni{}{t}, \\
	\label{LP:PowerLimits}
	& \pgmin\leq \pg_{t}  \leq \pgmax, \\ 
	\label{LP:energy}
	& \bepsilonminS \leq \bepsilon_t \leq \bepsilonmaxS,\\
	\label{LP:ramp}
	& \pni{, \text{off}}{g,t} \leq \pgrdown,\quad \pni{, \text{on}}{g,t}  \leq \pgrup .
\end{align}    
\end{subequations}    
\end{linenomath}

The objective~\eqref{LP:obj} is to minimize the energy cost, where the cost coefficients $\bfc^f$ represent marginal cost and approximate start-up costs of each conventional generation unit $g\in\bfG$.
The power injection variables $\pg=\bmat{\pgen, \ps}$ consists not only of the conventional generator outputs $\pgen$ but also includes the injections $\ps$ incurred by the storage devices.
The conventional power output is represented recursively with respect to the previous time instance and the power increment $\pni{, \text{on}}{g,t}$ and decrement $\pni{, \text{off}}{g,t}$ in the current time period, as expressed in~\eqref{LP:pg}. Considering this representation, minimum up-/down-time and generation ramp constraints can be easily approximated by additional linear constraints. The demand balance constraint~\eqref{LP:balance} states that the sum of all generation components (power plants, net import, and storage discharge) should be equal to the sum of all load components (demand and storage charging) for all time instances $t \in \bfT$. The net import $\bfn^v_{t} $ is simply a sum of the power imports and exports for the given zone of interest. Additional constraints are imposed for the links between the zones, such as maximum capacity or flow-based constraints~\cite{flowCoupling}.

Energy storage devices are modeled using  charging and discharging efficiencies and technical limitations of the state of charge, similar to models in~\cite{beltistos,most}. 
%
$\Ns$ energy storage units are considered, where the vector of the storage power injections consists of discharging and charging injections,
\begin{linenomath}
\begin{equation}
\ps = \bmat{ \psdni{}{1}, \ldots ,\psdni{}{\Ns},  \pscni{}{1},  \ldots , \pscni{}{\Ns}}.
\end{equation}
\end{linenomath}
%The composite vector considering also the generator power injections is thus $\pg = \pmat{\pg_{gen},\ \ps}$.
The evolution of the state of charge levels $\bepsilon_t \in\R{\Ns}$ follows the update equation
\begin{linenomath}
\begin{align}
\label{Eq:linup}
% \bepsilon^{n+1} = \bepsilon^n + \delta t \; \Bs \; \psn \quad n = 0,1,\ldots,N-1,
\bepsilon_{t} = \bepsilon_{t-1} + \Bs \; \psn \quad t = 1,\ldots,N,
\end{align}
\end{linenomath}
and introduces a coupling between the individual time periods. The energy level in each period needs to honor the storage capacity, as expressed by the constraint \eqref{LP:energy}.
The initial storage level is denoted $\bepsilon_0$ and the constant matrix $\Bs \in\R{\Ns\times2\Ns}$ models discharging and charging efficiencies of the storage devices,
\begin{linenomath}
\begin{align}
\Bs  = -\delta t
\pmat{\eta_{\text{d},1}^{-1}&  & &\eta_{\text{c},1} & &  \\
	%           & & -\eta_{d,2}^{-1}& \eta_{c,2}^{-1} & & & & \\
	%            & & & & \ddots & \ddots & & \\
	& \ddots&  &  &\ddots & \\
	& & \eta_{\text{d},\Ns}^{-1}& & & \eta_{\text{c},\Ns} }
\end{align}
\end{linenomath}
with the discharging and charging efficiencies $\eta_{\text{d},i}$ and $\eta_{\text{c},i}$, $i = 1,2,\ldots,\Ns$.
%The vector of storage levels has to respect the storage level bounds at each time period $n$, $\bepsilonminS \leq \bepsilon_n \leq \bepsilonmaxS$.
%The vector of storage levels has to satisfy two types of constraints.  First, the storage level is bounded  at each time period $n$ by $\bepsilonminS \leq \bepsilon_n \leq \bepsilonmaxS$.  Second, the storage level at the end of the dispatch horizon $N$ should match its initial value in order to avoid depletion of the storage and to obtain a solution cost that is independent from changes in storage energy,
%\begin{equation}
% \label{Eq:StoragesConstraint}
%   \bepsilon_N =  \bepsilon_{0}.
%\end{equation}
%The linear inequality constraints introduced by storage devices can be written in matrix form involving powers from all storage devices, generators, and time periods as 
%\begin{equation}\label{Eq:storages_N}
%%\underbrace{ \pmat{\bepsilonminS\\\bepsilonminS\\\vdots 
%%		\\ \bepsilonminS}}_{\bepsilonmin}
%%\leq
%\underbrace{ \pmat{\bepsilon_0\\ \bepsilon_0\\ \vdots\\ \bepsilon_0  }}_{\Ezero} +
%\underbrace{
%	\pmat{\Bs &        &        &        \\
%		\Bs &     \Bs &        &        \\
%		\vdots & \vdots & \ddots &        \\
%		\Bs &     \Bs & \cdots & \Bs}
%}_{\E}
%\underbrace{\pmat{\ps_1\\ \ps_2 \\ \vdots \\ \ps_N}}_{\ps},
%%\leq
%%\underbrace{ \pmat{\bepsilonmaxS\\ \bepsilonmaxS\\ \vdots\\ \bepsilonmaxS }}_{\bepsilonmax}.
%\end{equation}
%\begin{equation}
%\bepsilonmin \leq \Ezero + \E \ps \leq \bepsilonmax.
%\end{equation}

%Flow based market coupling allocates cross-border flows considering power transfer distribution factors (PTDFs) which describe the sensitivity of a change in import/export at a particular country. The PTDF matrix and the remaining available margin (RAM) determine the feasible transmission region at any given point in time. On a daily basis, the Capacity Auctioning Service Company (CASC) gives information about maximum bilateral exchanges, minimum and maximum net positions and PTDFs for the day-ahead market \cite{flowCoupling}.

==> 05experiments-derivative.tex <==
\section{Numerical Experiments - Derivative-based Sensitivity}

\subsubsection{Independent Parameters \label{sec:der_independent}}
The derivative-based indices are first studied without considering any parameter correlations, assuming their complete independence. The sensitivities are computed by evaluating analytical derivatives of the surrogate polynomial model. In practice, the finite differences (FD) are usually used to compute the derivatives.The limitation of the FD is that they cannot consider any parameter interaction, nor their correlation. But since in this experiment no correlation is assumed, FD is used as a reference value to assess the quality of the derivative obtained from the surrogate model.  Apart from the approximation errors, both approaches should provide equivalent results. The error in the FDs stems from approximating the slope of the model response in the direction of a given parameter by considering a small model perturbation $\delta$. On the other hand, the analytical derivative of the surrogate model can be computed exactly, but the surrogate model only approximates the true model response, thus the slope might not represent the slope of the true model.

The FD and PCE-based derivatives with respect to a set of fuels for model output shown in Fig.~\ref{fig:price_zone_21} are shown in Fig.\ref{fig:derivatives_zone_21}. The FDs approximation with $\delta = 5\%$ was used, while the second order polynomial expansion was used to construct the surrogate model. As noted above, the results are not identical due to inherent numerical and approximation errors in both approaches, but the sensitivity indices follow a similar trend.

\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_der_price_gas_zone_21.pdf}
        \caption{Gas price sensitivity.}
        \label{fig:derivatives_zone_21_gas}
    \end{subfigure}
    %
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_der_price_coal_zone_21.pdf}
        \caption{Coal price sensitivity.}
        \label{fig:derivatives_zone_21_coal}
    \end{subfigure}
    %
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_der_price_emission_zone_21.pdf}
        \caption{Emission price sensitivity.}
        \label{fig:derivatives_zone_21_em}
    \end{subfigure}
    \caption{Derivative-based indices considering independent parameters.}
    \label{fig:derivatives_zone_21}
\end{figure}


\subsubsection{Parameter Dependency \label{sec:derl_dependency}}

Similar to the experiment in Sec.~\ref{sec:sobol_dependency}, the covariance matrix \eqref{eq:covariance} was used with the same permutation vector. The resulting derivative-based sensitivity indices are shown in Fig.\ref{fig:derivatives_dep_zone_21}. As expected, the full sensitivity index for the gas shown in Fig.~\ref{fig:derivatives_dep_zone_21_gas} parameter was increased compared to the independent case, including all the correlated interaction with other two parameters. On the contrary, the marginal and independent indices of the other parameters were cleared from the correlated contributions with gas, thus the overall sensitivity index is reduced compared to the base case, as shown in Figs.~\ref{fig:derivatives_dep_zone_21_coal} and ~\ref{fig:derivatives_dep_zone_21_em}.  

\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_dep_der_price_gas_zone_21.pdf}
        \caption{Gas price sensitivity.}
        \label{fig:derivatives_dep_zone_21_gas}
    \end{subfigure}
    %
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_dep_der_price_coal_zone_21.pdf}
        \caption{Coal price sensitivity.}
        \label{fig:derivatives_dep_zone_21_coal}
    \end{subfigure}
    %
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_dep_der_price_emission_zone_21.pdf}
        \caption{Emission price sensitivity.}
        \label{fig:derivatives_dep_zone_21_em}
    \end{subfigure}
    \caption{Derivative-based indices considering correlated parameters.}
    \label{fig:derivatives_dep_zone_21}
\end{figure}

\subsubsection{Parameter Dependency - Increasing Correlation  \label{sec:derl_dependency_inc}}

\subsubsection{Convergence \label{sec:der_convergence}}
Convergence of the PCE with respect to the polynomial order is shown in Fig.~\ref{fig:derivatives_zone_21_convergence}. 


\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_der_price_gas_zone_21_convergence.pdf}
        \caption{Gas price sensitivity.}
        \label{fig:derivatives_zone_21_gas_convergence}
    \end{subfigure}
    %
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_der_price_coal_zone_21_convergence.pdf}
        \caption{Coal price sensitivity.}
        \label{fig:derivatives_zone_21_coal_convergence}
    \end{subfigure}
    %
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_der_price_emission_zone_21_convergence.pdf}
        \caption{Emission price sensitivity.}
        \label{fig:derivatives_zone_21_em_convergence}
    \end{subfigure}
    \caption{Convergence of derivative-based indices considering independent parameters.}
    \label{fig:derivatives_zone_21_convergence}
\end{figure}


==> 05experiments-variance.tex <==
\section{Numerical Experiments - Variance-based Sensitivity}

This section presents a series of experiments  related to the variance-based Sobol indices associated with the European energy market model presented in Sec.~\ref{sec:LPmodel}.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=1\textwidth]{figures/mps_derivatives/SAmodel_zone_21_PO_3.pdf}
    \caption{Model output.}
    \label{fig:price_zone_21}
\end{figure}

\subsubsection{Independent Parameters \label{sec:sobol_independent}}
The variance-based Sobol indices are computed for the energy price in market zone 21 with respect to the underlying fuel prices, as shown in Fig.~\ref{fig:price_zone_21}.
In this case the correlation matrix $\mathcal{C}$ is an identity matrix, i.e. there is no correlation between the parameters. Note that the model variance at some time periods is near zero, thus the Sobol indices shown might be affected by the numerical errors. Note that the Sobol index is not defined in case the overall model variance is zero.

The Sobol indices are shown in Fig.~\ref{fig:sobol_independent}. The important parameters which explain most of the model variance are the gas and emission prices, while the model ouput is relatively not influenced by the coal price, except for a single hour where the situation inverts.
The difference of the first and total order indices are usually below 10\%, indicating there are no important high order parameter interactions. Since there are no large high order interactions, the first order Sobol indices add up close to one. 
%The first order Sobol index of the $\kappa$ parameter, shown in Fig.~\ref{fig:coffee_independent_first}, is the most influential in the first 75 minutes, while the ambient temperature dominates in the remaining time. After reaching near equilibrium, i.e. the ambient and the coffee cup temperature difference is less than $\approx  0.1^\circ\text{C}$, the ambient temperature parameter explains nearly all of the output variance as shown in Fig.~\ref{fig:price_zone_21}. Intuitively, this is a reasonable situation since the end state of the coffee cup after reaching the equilibrium is the environment temperature. 

\begin{figure}[ht!]
    \centering
    \includegraphics[width=1\textwidth]{figures/mps_derivatives/SAerror_sobol_zone_21.pdf}
    \caption{Sobol indices considering independent parameters.}
    \label{fig:sobol_independent}
\end{figure}



\subsubsection{Parameter Dependency \label{sec:sobol_dependency}}
Next, the correlation matrix $\mathcal{C}$ is modified, such that the off-diagonal elements are no longer zero, indicating parameter correlation. In the following numerical experiment, the covariance matrix $\C$ was used,
\begin{equation}
    \label{eq:covariance}
    \C = \begin{pmatrix}
        0.001036051621, & 0.000683135802, & 0.000762425637\\
        0.000683135802, & 0.000965909304, & 0.000384625925\\
        0.000762425637, & 0.000384625925, & 0.001953453051
    \end{pmatrix}
\end{equation}
The permutation $P = (\text{gas}, \text{coal}, \text{emission})$ was used for the correlation. Thus full index of the gas parameter, marginal index for coal and independent index for emission are obtained, as detailed in Tab.~\ref{tab:indices}.
%

The Sobol indices for correlated parameters are shown in Fig.~\ref{fig:sobol_dependent}, while their error relative to the baseline experiment with independent parameters is shown in Fig.~\ref{fig:sobols_dep_zone_21}.
As shown in Fig.~\ref{fig:sobols_dep_zone_21_gas}, the full order index of the gas parameter (i.e. gas is at the first position in the permutation vector), the contribution of this parameter to the output variance is increased compared to the independent case. When the independent index is considered for the emission parameter ( i.e. emission is last  in the permutation), the effect of the correlation with other parameters  is removed and consequently, the index is proportionally reduced, as shown in Fig.~\ref{fig:sobols_dep_zone_21_em}. Similar holds for the coal parameter in Fig.~\ref{fig:sobols_dep_zone_21_coal}, which was reduced by the correlation with the gas parameter.

Removal of the correlation contribution decreases the value of the sensitivity index. 
%The magnitude of the change is proportional to the difference in parameter indices (full vs. independent index). 
%{\color{red} TODO: add pie graph illustrating the idea below, sum of indices to 1 with overlapping corellated indices.}
This can be interpreted such that the portion of the output variance can be explained by both parameters simultaneously since they are correlated. It can be equally said that some output variance is explained either by one or the other parameter. In the extreme case of perfect correlation it is equivalent to say that the output variance is explained either by one or the other parameter, since the value of one parameter completely determines the value of the other.
%{\color{red} this can explain the behavior at t>125min, but what about  the offset of 0.2 in the time range between 25-75min? The correlated indices are never as in the base independent case.} 

\begin{figure}[ht!]
    \centering
    \includegraphics[width=1\textwidth]{figures/mps_derivatives/SAerror_dep_sobol_zone_21.pdf}
    \caption{Sobol indices considering correlated parameters.}
    \label{fig:sobol_dependent}
\end{figure}

\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_sobol_price_gas_zone_21.pdf}
        \caption{Gas price sensitivity.}
        \label{fig:sobols_dep_zone_21_gas}
    \end{subfigure}
    %
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_sobol_price_coal_zone_21.pdf}
        \caption{Coal price sensitivity.}
        \label{fig:sobols_dep_zone_21_coal}
    \end{subfigure}
    %
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_sobol_price_emission_zone_21.pdf}
        \caption{Emission price sensitivity.}
        \label{fig:sobols_dep_zone_21_em}
    \end{subfigure}
    \caption{First order Sobol indices considering correlated parameters.}
    \label{fig:sobols_dep_zone_21}
\end{figure}


%It is also interesting to observe the complement of the indices to one, shown in  Fig.~\ref{fig:coffee_dependent_complement}. Consider the full index of the $\kappa$ parameter, then its complement to one explains the output variance contributed by the other parameter alone without its correlated contribution with $\kappa$. In case of the two parameters, this complement is the independent Sobol index of the $T_{env}$ parameter, as shown in Fig.~\ref{fig:coffee_dependent_complement}a. In general case with a set of $P$ parameters, complement of the full index of the parameter $i$ explains the amount of variance contributed by the remaining $P\setminus \{i\}$ parameters without their correlated contribution with $i$.
%
%A similar relationship is observed between the complement of the full index of $T_{env}$ and independent index of $\kappa$ in Fig.~\ref{fig:coffee_dependent_complement}b. Note the presence of a numerical error in this case, in order to eliminate it, the indices should be computed with higher order polynomials in the PCE analysis or larger number of samples in case of the QMC method.
%%
%Similarly, Fig.~\ref{fig:coffee_dependent_complement}c-d illustrate the relationship between the complement of the independent indices and the full indices of the other parameter.
%
%\begin{figure}[ht!]
%    \centering
%    \includegraphics[width=1\textwidth]{figures/coffee/SAcomplement.pdf}
%    \caption{Complementary behaviors of the indices.}
%    \label{fig:coffee_dependent_complement}
%\end{figure}
%
\subsubsection{Parameter Dependency - Increasing Correlation \label{sec:sobol_dependency_inc}}
%Next, the correlation matrix $\mathcal{C}$ is modified, such that the off-diagonal elements $\rho_{12}$ are increased in increments $0.2$, ranging from zero all the way to one (i.e. from no correlation up to perfect correlation).
%%
%The study of the First order Sobol indices is first performed considering the permutation $(\kappa, T_{env})$, which enables one to compute Full Sobol index for $\kappa$ and an independent index for $T_{env}$ shown in Fig.~\ref{fig:coffee_dependent_corr}.
%The permutation $(T_{env}, \kappa)$ is used afterwards, to compute Independent Sobol index for $\kappa$ and the Full index for $T_{env}$ shown in Fig.~\ref{fig:coffee_dependent_corr1}.
%
%It can be observed that as the correlation increases, the Full index of $\kappa$ at $t>125min$ in Fig.~\ref{fig:coffee_dependent_kappa_corr} is gradually increasing, while at the same time the independent index of the other parameter in Fig.~\ref{fig:coffee_dependent_tenv_corr} proportionally decreases. This reflects the fact that due to the correlation, the Full index $\kappa$ becomes gradually more significant due to its correlation with the $T_{env}$ parameter, not because of the parameter $\kappa$ itself. On the other hand, the amount of the variance explained by $T_{env}$ alone decreases with increasing correlation, because of its interaction with $\kappa$.
%%
%In the limit situation when $\rho_{12}=1$, the parameters alone become insignificant and all of the variance is explained by their correlated interaction. Note that the Independent index of both parameters is zero near the end of the time domain (Fig.~\ref{fig:coffee_dependent_tenv_corr} and~\ref{fig:coffee_dependent_kappa_corr1}),
%while the Full index is one (Fig.~\ref{fig:coffee_dependent_kappa_corr} and ~\ref{fig:coffee_dependent_tenv_corr1}).
%
%\begin{figure}[ht!]
%    \centering
%    \begin{subfigure}[b]{0.85\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figures/coffee/SAerror_kappa_corr.pdf}
%        \caption{First order Full index of the $\kappa$ parameter.}
%        \label{fig:coffee_dependent_kappa_corr}
%    \end{subfigure}
%    
%    \begin{subfigure}[b]{0.85\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figures/coffee/SAerror_t_env_corr.pdf}
%        \caption{First order Independent index of the $T_{env}$ parameter.}
%        \label{fig:coffee_dependent_tenv_corr}
%    \end{subfigure}
%    \caption{Sobol indices considering dependent parameters with increasing correlation $\rho_{12}$ and  permutation $(\kappa, T_{env})$, error relative to the independent indices.}
%    \label{fig:coffee_dependent_corr}
%\end{figure}
%
%\begin{figure}[ht!]
%    \centering
%    \begin{subfigure}[b]{0.85\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figures/coffee/SAerror_kappa_corr1.pdf}
%        \caption{First order Independent index of the $\kappa$ parameter.}
%        \label{fig:coffee_dependent_kappa_corr1}
%    \end{subfigure}
%    
%    \begin{subfigure}[b]{0.85\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figures/coffee/SAerror_t_env_corr1.pdf}
%        \caption{First order Full index of the $T_{env}$ parameter.}
%        \label{fig:coffee_dependent_tenv_corr1}
%    \end{subfigure}
%    \caption{Sobol indices considering dependent parameters with increasing correlation $\rho_{12}$ and  permutation $(T_{env},\kappa)$, error relative to the independent indices.}
%    \label{fig:coffee_dependent_corr1}
%\end{figure}

\subsubsection{Convergence \label{sec:sobol_convergence}}
Convergence of the PCE with respect to the polynomial order is shown in Fig.~\ref{fig:sobols_dep_zone_21_convergence}. 
A rather arbitrary value of $0.05$ is frequently used in the sensitivity analysis literature for distinguishing important from unimportant parameters~\cite{GSA-cutoff}, thus similar idea can be applied to declaring a method to converge. If the absolute error between the indices is below the threshold of significance $0.05$, the method can be considered to have converged.

%The PCE method is run with an increasing polynomial order, ranging from 2nd to 7th order. Figure~\ref{fig:coffee_converg_kappa_pce} illustrates that the indices computed by the PCE method differ from the reference value of the QMC by less than $0.05$ for polynomial order three and higher orders. For the fourth polynomial order, the error  is below $0.01$. For practical purposes the analysis can be run with third of fourth order polynomials.

\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_sobol_price_gas_zone_21_convergence.pdf}
        \caption{Gas price sensitivity.}
        \label{fig:sobols_dep_zone_21_gas_convergence}
    \end{subfigure}
    %
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_sobol_price_coal_zone_21_convergence.pdf}
        \caption{Coal price sensitivity.}
        \label{fig:sobols_dep_zone_21_coal_convergence}
    \end{subfigure}
    %
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mps_derivatives/SAerror_sobol_price_emission_zone_21_convergence.pdf}
        \caption{Emission price sensitivity.}
        \label{fig:sobols_dep_zone_21_em_convergence}
    \end{subfigure}
    \caption{Convergence of first order Sobol indices considering independent parameters.}
    \label{fig:sobols_dep_zone_21_convergence}
\end{figure}

%The convergence of the QMC method is studied, which is later used as a reference value for the PCE method. The QMC method is run with an increasing number of samples, and the resulting first order indices are shown in Fig.~\ref{fig:coffee_converg_qmc}. The absolute error between the indices is well below the threshold of significance $0.05$, thus the method is considered to have converged.
%The rather arbitrary value of $0.05$ is frequently accepted for this type of analysis for distinguishing important from unimportant parameters~\cite{GSA-cutoff}, thus similar idea can be applied to declaring a method to converge.
%
%\begin{figure}[ht!]
%    \centering
%    \begin{subfigure}[b]{0.85\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figures/coffee/SAerror_kappa_converg_qmc.pdf}
%        \caption{First order index of the $\kappa$ parameter.}
%        \label{fig:coffee_converg_kappa_qmc}
%    \end{subfigure}
%    
%    \begin{subfigure}[b]{0.85\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figures/coffee/SAerror_tenv_converg_qmc.pdf}
%        \caption{First order index of the $T_{env}$ parameter.}
%        \label{fig:coffee_converg_tenv_qmc}
%    \end{subfigure}
%    \caption{Convergence of QMC method for Sobol indices considering dependent parameters using permutation $(T_{env},\kappa)$.}
%    \label{fig:coffee_converg_qmc}
%\end{figure}
%
%The PCE method is run with an increasing polynomial order, ranging from 2nd to 7th order. Figure~\ref{fig:coffee_converg_kappa_pce} illustrates that the indices computed by the PCE method differ from the reference value of the QMC by less than $0.05$ for polynomial order three and higher orders. For the fourth polynomial order, the error  is below $0.01$. For practical purposes the analysis can be run with third of fourth order polynomials. The error in the initial point is attributed to the fact that the variance in this point is zero and the variance-based Sobol indices are not defined, thus the error is meaningless here.
%
%\begin{figure}[ht!]
%    \centering
%    \begin{subfigure}[b]{0.85\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figures/coffee/SAerror_kappa_converg_pce.pdf}
%        \caption{First order index of the $\kappa$ parameter.}
%        \label{fig:coffee_converg_kappa_pce}
%    \end{subfigure}
%    
%    \begin{subfigure}[b]{0.85\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figures/coffee/SAerror_tenv_converg_pce.pdf}
%        \caption{First order index of the $T_{env}$ parameter.}
%        \label{fig:coffee_converg_tenv_pce}
%    \end{subfigure}
%    \caption{Convergence of PCE method for Sobol indices considering dependent parameters using permutation $(T_{env},\kappa)$.}
%    \label{fig:coffee_converg_pce}
%\end{figure}


==> figures/greasy/slowdownCSCS.tex <==
\begin{tikzpicture}

% COLORS 
%4-class OrRd Tokyo SIAM PP18
\definecolor{mycolor0}{HTML}{2B83BA}
\definecolor{mycolor1}{HTML}{D7301F}
\definecolor{mycolor2}{HTML}{FC8D59}
\definecolor{mycolor3}{HTML}{FDCC8A}
\definecolor{mycolor4}{HTML}{FEF0D9}
\definecolor{mycolor5}{HTML}{FEF0D9}
\definecolor{mycolor6}{HTML}{009933}

\pgfplotstableread{figures/greasy/cscs.dat}\data;


\begin{axis}[
width=.9\columnwidth, height=4.0cm, 
% ybar,
% bar width=3.5pt, 
ymin=0,
ymax=126,
xmin=0,xmax=38,
axis lines*=left, 
ymajorgrids, yminorgrids,
% xtick=data,
% xticklabels from table={\ipresults}{numProcs},
%xtick={1,16,32,48,64,80,96,112,128},
xtick={1,4,8,12,16,20,24,28,32,36},
% enlarge x limits=0.05,
xticklabel style={align=center, rotate=0, anchor=north, font=\scriptsize},
ytick={20,40,60,80,100,120},
xticklabel style={font=\scriptsize},
yticklabel style={font=\scriptsize},
xlabel style={font=\scriptsize},
ylabel style={font=\scriptsize},
xlabel={Number of concurrent LP solves $c$},
ylabel={Measured $ t_{avg}^c$ (s)},
clip=false,
% legend style={at={(.4,1.0)},fill=white,legend cell align=left,align=right,draw=white!85!black,font=\scriptsize,legend columns=1},
]
%\addplot[smooth,mycolor1,thick,mark=*,mark size=1.5pt] table[x=numProcs, y=ipont_tc_ave] {\data}; \label{ip}
\addplot[smooth,mycolor0,thick,mark=o,mark size=1.5pt] table[x=numProcs, y=simplex_tc_ave] {\data}; \label{simplexCSCS}
% \addlegendentry{Dual Simplex}
\end{axis}

\begin{axis}[
width=.9\columnwidth, height=4.0cm, 
% ybar,
% bar width=3.5pt, 
ymin=1800,
ymax=6100,
xmin=0,xmax=38,
axis lines*=right, 
axis x line=none,
% ymajorgrids, 
yminorgrids,
% xtick=data,
% xticklabels from table={\ipresults}{numProcs},
%xtick={1,16,32,48,64,80,96,112,128},
% enlarge x limits=0.05,
% xticklabel style={align=center, rotate=0, anchor=north, font=\scriptsize},
ytick={2000, 3000, 4000, 5000, 6000},
% xticklabel style={font=\scriptsize},
yticklabel style={font=\scriptsize},
% xlabel style={font=\scriptsize},
ylabel style={font=\scriptsize},
% xlabel={$t_1000$},
ylabel={$t_{1000}$  (s)},
clip=true,
legend style={at={(0.999,1.12)},fill=none,legend cell align=left,align=right,draw=none,font=\scriptsize,legend columns=2},
]
%\addlegendimage{/pgfplots/refstyle=ip}\addlegendentry{IP $t^c_{avg}$}
\addlegendimage{/pgfplots/refstyle=simplexCSCS}\addlegendentry{Measured $t^c_{avg}$}

%\addplot[smooth,mycolor1,thick,dash dot dot] table[x=numProcs, y=t_n_ipoint] {\data};
%\addlegendentry{IP $t_{1000}$}
\addplot[smooth,mycolor1,thick,dashed] table[x=numProcs, y=t_n_simplex] {\data};
\addlegendentry{Estimated $t_{1000}$}

%\addplot[smooth,mycolor1,thick, mark=x] table[x=numProcs_actual, y=t_actual] {\data};
%\addlegendentry{Measured $t_{1000}$}
\end{axis}

\end{tikzpicture}


==> figures/greasy/slowdownDXT.tex <==
\begin{tikzpicture}

% COLORS 
%4-class OrRd Tokyo SIAM PP18
\definecolor{mycolor0}{HTML}{2B83BA}
\definecolor{mycolor1}{HTML}{D7301F}
\definecolor{mycolor2}{HTML}{FC8D59}
\definecolor{mycolor3}{HTML}{FDCC8A}
\definecolor{mycolor4}{HTML}{FEF0D9}
\definecolor{mycolor5}{HTML}{FEF0D9}
\definecolor{mycolor6}{HTML}{009933}

\pgfplotstableread{figures/greasy/dxt.dat}\data;


\begin{axis}[
width=.9\columnwidth, height=4.0cm, 
% ybar,
% bar width=3.5pt, 
ymin=0,
ymax=126,
xmin=-3,xmax=132,
axis lines*=left, 
ymajorgrids, yminorgrids,
% xtick=data,
% xticklabels from table={\ipresults}{numProcs},
xtick={1,16,32,48,64,80,96,112,128},
% enlarge x limits=0.05,
xticklabel style={align=center, rotate=0, anchor=north, font=\scriptsize},
ytick={20,40,60,80,100,120},
xticklabel style={font=\scriptsize},
yticklabel style={font=\scriptsize},
xlabel style={font=\scriptsize},
ylabel style={font=\scriptsize},
xlabel={Number of concurrent LP solves $c$},
ylabel={Measured $ t_{avg}^c$ (s)},
clip=false,
% legend style={at={(.4,1.0)},fill=white,legend cell align=left,align=right,draw=white!85!black,font=\scriptsize,legend columns=1},
]
%\addplot[smooth,mycolor1,thick,mark=*,mark size=1.5pt] table[x=numProcs, y=ipont_tc_ave] {\data}; \label{ip}
\addplot[smooth,mycolor0,thick,mark=o,mark size=1.5pt] table[x=numProcs, y=simplex_tc_ave] {\data}; \label{simplex}
% \addlegendentry{Dual Simplex}
\end{axis}

\begin{axis}[
width=.9\columnwidth, height=4.0cm, 
% ybar,
% bar width=3.5pt, 
ymin=400,
ymax=1030,
xmin=-3,xmax=132,
axis lines*=right, 
axis x line=none,
% ymajorgrids, 
yminorgrids,
% xtick=data,
% xticklabels from table={\ipresults}{numProcs},
xtick={1,16,32,48,64,80,96,112,128},
% enlarge x limits=0.05,
% xticklabel style={align=center, rotate=0, anchor=north, font=\scriptsize},
ytick={500,600,700,800,900,1000},
% xticklabel style={font=\scriptsize},
yticklabel style={font=\scriptsize},
% xlabel style={font=\scriptsize},
ylabel style={font=\scriptsize},
% xlabel={$t_1000$},
ylabel={$t_{1000}$  (s)},
clip=true,
legend style={at={(0.95,1.12)},fill=none,legend cell align=left,align=right,draw=none,font=\scriptsize,legend columns=2},
]
%\addlegendimage{/pgfplots/refstyle=ip}\addlegendentry{IP $t^c_{avg}$}
\addlegendimage{/pgfplots/refstyle=simplex}\addlegendentry{Measured $t^c_{avg}$}

%\addplot[smooth,mycolor1,thick,dash dot dot] table[x=numProcs, y=t_n_ipoint] {\data};
%\addlegendentry{IP $t_{1000}$}
\addplot[smooth,mycolor1,thick,dashed] table[x=numProcs, y=t_n_simplex] {\data};
\addlegendentry{Estimated $t_{1000}$}

\addplot[smooth,mycolor1,thick, mark=x] table[x=numProcs_actual, y=t_actual] {\data};
\addlegendentry{Measured $t_{1000}$}
\end{axis}

\end{tikzpicture}

